Sampling Agnostic Feature Representation for Long-Term Person Re-identification

Person re-identification is a problem of identifying individuals across non-overlapping cameras. Although remarkable progress has been made in the re-identification problem, it is still a challenging problem due to appearance variations of the same person as well as other people of similar appearance. Some prior works solved the issues by separating features of positive samples from features of negative ones. However, the performances of existing models considerably depend on the characteristics and statistics of the samples used for training. Thus, we propose a novel framework named sampling independent robust feature representation network (SirNet) that learns disentangled feature embedding from randomly chosen samples. A carefully designed sampling independent maximum discrepancy loss is introduced to model samples of the same person as a cluster. As a result, the proposed framework can generate additional hard negatives/positives using the learned features, which results in better discriminability from other identities. Extensive experimental results on large-scale benchmark datasets verify that the proposed model is more effective than prior state-of-the-art models.

==> 3_4_total_loss.tex <==
\subsection{Total Loss}

The cross-entropy loss $L_{id}$ and triplet loss $L_{tri}$ are also used to optimize the network. Additionally, $L_{CAM}$ also used for generate CAM. Then, $L_{id}$, $L_{tri}$ and $L_{CAM}$: 
\begin{align}\label{eq:id_tri_loss}
    \begin{array}{c}
        L_{id} = -y_i\cdot\log{p\left(f_\alpha\right)} - y_i\cdot\log{p\left(f_\beta\right)}, \vspace{0.3cm} \\
        L_{tri} = \max\left(0, m + ||f_\alpha - f_\alpha^+||_2 - ||f_\alpha - f_\alpha^-||_2\right), \vspace{0.3cm} \\
        L_{CAM} = -y_i\cdot\log{p\left(f_b\right)}
    \end{array}
\end{align}
where $p\left(\cdot\right)$ is predicted probability, $m$ is the margin and $f_b$ is denoted backbone features. Finally, the overall loss can be written as:
\begin{align}\label{eq:total_loss}
    L_{total} = \lambda_{rep}L_{rep} + \lambda_{recon}L_{recon} + \lambda_{id}L_{id} + \lambda_{tri}L_{tri}, 
\end{align}
where $\lambda_{rep}$, $\lambda_{recon}$, $\lambda_{id}$, and $\lambda_{tri}$ are weights for loss function. 


==> f_cluster_mix.tex <==
\begin{figure*}[!h]
    \begin{minipage}{1.0\linewidth}
    \centering
    \renewcommand{\tabcolsep}{1mm}
    \begin{tabular}{@{}ccc|ccc c@{}}
        \multicolumn{3}{c|}{Celeb-reID}& \multicolumn{3}{c}{LTCC}\\
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/05_rep_40_4.png} & \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/10_nrep_40_4.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/15_nrep_40_4.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_rep05.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_nrep50.png} &
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_nrep100.png} & 
        \multirow{4}{*}{\includegraphics[scale=0.4]{figs/tsne_cluster/t_SNE_label.png}}\\
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/05_rep_40_4.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/10_rep_40_4.png} &
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/15_rep_40_4.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_rep05.png} &
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_rep50.png} & 
        \includegraphics[width=0.15\textwidth]{figs/tsne_cluster/LTCC_rep100.png} & \\
        $5^{\textrm{th}}$ epoch & $10^{\textrm{th}}$ epoch & $15^{\textrm{th}}$ epoch & $5^{\textrm{th}}$ epoch & $50^{\textrm{th}}$ epoch & $100^{\textrm{th}}$ epoch & \\
    \end{tabular}     
    \end{minipage}
    \caption{Visualization of the t-SNE~\cite{van2008visualizing} scatter plots on Celeb-reID~\cite{Huang_2020_TCSVT} and LTCC~\cite{qian2020long} datasets. The 11 identities are randomly selected, with 160 samples from each identity in the galleries of both datasets. The figures in the first row are the clusters of the selected identities using the model trained without sample-independent maximum discrepancy loss $\mathcal{L}_{sim}$. The figures in the second row are the clusters using the model trained with $\mathcal{L}_{sim}$. As demonstrated in the figure, the sample-independent maximum discrepancy loss with classification losses performs better clustering than without it. Note that the mAP and rank-1 accuracy~(mAP/rank-1) at the $15^{\textrm{th}}$ epoch are $(12.7\% /53.4\%)$ for the model without $\mathcal{L}_{sim}$ and $(13.4\% / 55.1\%$ for the model with $\mathcal{L}_{sim}$ on Celeb-reID. The mAP and rank-1 accuracy~(mAP/rank-1) at the $15^{\textrm{th}}$ epoch are $(45.0\% / 74.9\%)$ for the model without $\mathcal{L}_{sim}$ and $(45.3\% /74.9\%)$ for the model with $\mathcal{L}_{sim}$ on LTCC. \vspace{0.5cm}} 
    \label{fig:tsne_cluster} 
    \begin{minipage}{1.0\linewidth}
      \centering
    \begin{tabular}{@{}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}|c@{~}c@{~}c@{~}c@{~}c@{~}}
    \parbox[t]{4mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Identity irrelevant $\xleftarrow{\makebox[4cm]{}}$~~~~~~}}} \hspace{0.2cm}
    & 
    \multicolumn{10}{l}{$\xrightarrow{\makebox[4cm]{}}$ Identity relevant} \vspace{0.2cm}
    \\
    & & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/0.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/1.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/2.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/3.png} &
    &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/0.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/1.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/2.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/3.png} 
    \\
    &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/0.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/00.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/01.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/02.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/03.png} &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/0.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc00.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc01.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc02.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc03.png}
    \\
    &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/1.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/10.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/11.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/12.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/13.png} &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/1.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc10.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc11.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc12.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc13.png}
    \\
    &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/2.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/20.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/21.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/22.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/23.png} &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/2.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc20.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc21.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc22.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc23.png}
    \\
    &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/3.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/30.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/31.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/32.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/celeb/33.png} &
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/3.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc30.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc31.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc32.png} & 
    \includegraphics[width=0.05\textwidth]{figs/mix_imgs/prcc/prcc33.png} \\
    & \multicolumn{5}{c|}{Celeb-reID} & \multicolumn{5}{c}{PRCC}
    \end{tabular}
    \end{minipage}
    \caption{Examples of the samples generated by the proposed feature augmentation module using Celeb-reID~\cite{Huang_2020_TCSVT} and PRCC~\cite{yang2019person} images. The reconstructed samples are augmented using the id-relevant features of persons in the each image of the first column and the id-irrelevant features of persons in the first row.}  \vspace{-0.2cm} \label{fig:mix}
\end{figure*}






==> f_mix_activation.tex <==
\begin{figure*}[!t]
    \begin{minipage}{1.0\linewidth}
    \centering
    \begin{tabular}{@{}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}|c@{~}c@{~}c@{~}c@{~}c@{~}}
    \parbox[t]{4mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Identity irrelevant $\xleftarrow{\makebox[4cm]{}}$~~~~~~}}} \hspace{0.2cm}
    & 
    \multicolumn{10}{l}{$\xrightarrow{\makebox[4cm]{}}$ Identity relevant} \vspace{0.3cm}
    \\
    & & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/0.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/1.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/2.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/3.png} &
    &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/0.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/1.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/2.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/3.png} 
    \\
    &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/0.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/00.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/01.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/02.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/03.png} &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/0.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc00.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc01.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc02.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc03.png}
    \\
    &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/1.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/10.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/11.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/12.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/13.png} &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/1.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc10.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc11.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc12.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc13.png}
    \\
    &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/2.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/20.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/21.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/22.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/23.png} &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/2.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc20.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc21.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc22.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc23.png}
    \\
    &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/3.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/30.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/31.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/32.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/celeb/33.png} &
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/3.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc30.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc31.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc32.png} & 
    \includegraphics[width=0.07\textwidth]{figs/mix_imgs/prcc/prcc33.png} \\
    & \multicolumn{5}{c|}{Celeb-reID} & \multicolumn{5}{c}{PRCC}
    \end{tabular}
    \vspace{0.3cm}
    \caption{Examples of the samples generated by the proposed feature augmentation module using Celeb-reID~\cite{Huang_2020_TCSVT} and PRCC~\cite{yang2019person} images. The reconstructed samples are augmented using the id-relevant features of persons in the each image of the first column and the id-irrelevant features of persons in the first row.  \vspace{1.5cm}}  \label{fig:mix}
    \end{minipage}
    %%%%% 
    \begin{minipage}{1.0\linewidth}
    \centering
    \begin{tabular}{@{}c@{~}c@{~}c@{~}|c@{~}c@{~}c@{~}|c@{~}c@{~}c@{}}
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/ltcc0.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/ltcc1.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/ltcc2.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/vcc0.jpg} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/vcc1.jpg} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/vcc2.jpg} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/21.jpg} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/81.jpg} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/310.jpg} \\ % \includegraphics[width=0.075\textwidth]{figs/activation/celeb/730.jpg} \\
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/cam0.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/cam1.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/ltcc/cam2.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/cam0.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/cam1.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/vcc/cam2.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/act0021.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/act0081.png} & 
    \includegraphics[width=0.075\textwidth]{figs/activation/celeb/act0310.png} \\
    % \includegraphics[width=0.075\textwidth]{figs/activation/celeb/act0730.png} \\
    \multicolumn{3}{c|}{LTCC} &  \multicolumn{3}{c|}{VC-Clothes} &  \multicolumn{3}{c}{Celeb-reID}
    \end{tabular}
    \caption{Examples of the feature activation mapping $E_{g}$ using LTCC~\cite{qian2020long}, VC-Clothes~\cite{wan2020person} and Celeb-reID~\cite{Huang_2020_TCSVT} dataset. The feature activation maps highlight the identity-specific discriminative regions.} \label{fig:activation}
    \end{minipage}
\end{figure*}

==> t_PRCC_LTCC.tex <==
\begin{table*}
    \centering
    \caption{Comparison results of PRCC \cite{Huang_2020_TCSVT} and LTCC \cite{qian2020long} datasets. The PRCC dataset is used in the cross-clothes setting, and the LTCC dataset is used standard and cloth-changing settings.}
    \label{tab:prcc_ltcc_scores}
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{PRCC\cite{Huang_2020_TCSVT}}& \multicolumn{4}{c}{LTCC\cite{qian2020long}} \\ \cline{2-7}
        & Rank1 & mAP & Rank1 & mAP & Rank1 & mAP \\ \hline \hline
        HACNN\cite{Li_2018_CVPR} & 21.8 & - & 60.2 & 26.7 & 21.6 & 9.3 \\
        PCB\cite{Sun_2018_ECCV} & 22.9 & - & 65.1 & 30.6 & 23.5 & 10.3 \\
        SPT\cite{yang2019person} & 34.4 & - & - & - & - & - \\
        CESD\cite{qian2020long} & - & - & 71.4 & 34.3 & 26.2 & 12.4 \\
        AFD-Net\cite{xuadversarial} & 42.8 & - & - & - & - & - \\
        FSAM\cite{hong2021fine} & 54.5 & - & 73.2 & 35.4 & 38.5 & 16.2 \\
        LaST\cite{shu2021large} & \textbf{57.5} & \textbf{54.7} & - & - & - & - \\
        
        \hline
        \textbf{Ours} & 50.5 & 49.6 & \textbf{74.9} & \textbf{45.3} & \textbf{40.1} & \textbf{23.1} \\
        
        \bottomrule
    \end{tabular}
\end{table*}


==> t_celeb_results.tex <==
\begin{table*}
    \centering
     \caption{Comparisons of performance on Celeb-reID and Celeb-reID-light datasets in terms of Rank-1/Rank-5 classification accuracy and mean average precision~(mAP).}
    \label{tab:celeb_scores}
    \begin{tabular}{l|ccc|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Celeb-reID\cite{Huang_2020_TCSVT}}& \multicolumn{3}{c}{Celeb-reID-light\cite{huang2019celebrities}} \\ \cline{2-7}
        & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP  \\ \hline \hline
        PCB\cite{Sun_2018_ECCV} & 37.1 & 57.0 & 8.2 & - & - & - \\
        MLFN\cite{Chang_2018_CVPR} & 41.4 & 54.7 & 6.0 & 10.6 & 31.0 & 6.3 \\
        IDE\cite{Zheng_2017_CVPR} & 42.9 & 56.4 & 5.9 & 10.5 & 24.8 & 5.3 \\
        %IDE+DenseNet121\cite{Zheng_2017_CVPR} & 42.9 & 56.4 & 5.9 & 10.5 & 24.8 & 5.3 \\
        ResNet-Mid\cite{yu2017devil} & 43.3 & 54.6 & 5.8 & 10.3 & 28.0 & 6.0 \\
        HACNN\cite{Li_2018_CVPR} & 47.6 & 63.3 & 9.5 & 16.2 & 42.8 & 11.5 \\
        MGN\cite{wang2018learning} & 49.0 & 64.9 & 10.8 & 21.5 & 47.4 & 13.9 \\
        CESD\cite{qian2020long} & 50.9 & 66.3 & 9.8 & - & - & - \\
        ReIDCaps\cite{Huang_2020_TCSVT} & 51.2 & 65.4 & 9.8 & 20.3 & 48.2 & 11.2 \\
        AFD-Net\cite{xuadversarial} & 52.1 & 66.1 & 10.6 & 22.2 & 51.0 & 11.3 \\
        LaST\cite{shu2021large} & 54.4 & - & 11.8 & - & - & - \\ \hline
        \textbf{Ours} & \textbf{55.2} & \textbf{69.3} & \textbf{13.4} & \textbf{32.5} & \textbf{67.6} & \textbf{19.2} \\
        \bottomrule
    \end{tabular}
\end{table*}

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lc@{}}
%    \toprule
%    Method & Frobnability \\
%    \midrule
%    Theirs & Frumpy \\
%    Yours & Frobbly \\
%    Ours & Makes one's heart Frob\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results.   Ours is better.}
%  \label{tab:example}
% \end{table}
